POSIT: Promotion of Semantic Item Tail via Adversarial Learning

In many recommendations, a handful of popular items (e.g., movies / television shows, news, etc.) can be dominant in recommendations for many users. However, we know that in a large catalog of items, users are likely interested in more than what is popular. The dominance of popular items may mean that users will not see items that they would probably enjoy. In this paper, we propose a technique to overcome this problem using adversarial machine learning. We define a metric to translate the user-level utility metric in terms of an advantage/disadvantage over items. We subsequently used that metric in an adversarial learning framework to systematically promote disadvantaged items. Distinctly, our method integrates a small-capacity model to produce semantically meaningful weights, leading to an algorithm that identifies and promotes a semantically similar item within the learning process. In the empirical study, we evaluated the proposed technique on three publicly available datasets and seven competitive baselines. The result shows that our proposed method not only improves the coverage, but also, surprisingly, improves the overall performance.

==> figures/tab_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{@{}cccccc@{}}
\toprule
\multirow{3}{*}{Dataset}       & \multirow{3}{*}{Method} & \multicolumn{4}{c}{Metric}                                                                                      \\ \cmidrule{3-6}
                               &                         & \multicolumn{1}{c}{NDCG@K}   & \multicolumn{3}{c}{Recall@K}                                                         \\ \cmidrule(lr){3-3} \cmidrule(lr){4-6}
                               &                         & \multicolumn{1}{c}{Top100} & \multicolumn{1}{c}{Top100} & \multicolumn{1}{c}{Top50} & \multicolumn{1}{c}{Top20} \\
\midrule
\multirow{7}{*}{Movie Lens}    & \system                    & \textbf{0.4214}              & \textbf{0.6369}                & \textbf{0.5244}                & \textbf{0.3928}               \\
                               & IPW                     & \textbf{0.4209}                       & \textbf{0.6364}                         & 0.5226                         & \textbf{0.3926}                        \\
                               & CVar                    & 0.4200                       & 0.6353                         & 0.5210                          & 0.3911                        \\
                               & Rerank                  & 0.4190                       & 0.6300                         & 0.5199                         & 0.3906                        \\
                               & EASE                    & 0.4199                       & 0.6356                         & 0.5209                         & 0.3906                        \\ 
                               & Causal                & 0.3695                  & 0.5599     &      0.4560   &   0.3411 \\
                               & Post & 0.3927 & 0.5525 & 0.4448 & 0.4118 \\
                               & MP                    &          0.1905              &        0.3300                &    0.2351                      &           0.1617              \\                               \cmidrule(lr){1-6}
\multicolumn{2}{c}{Standard Deviation}                 & \multicolumn{4}{c}{$\pm 0.0010$}\\
\midrule
\multirow{6}{*}{Netflix Prize} & \system                    & \textbf{0.3953}              & \textbf{0.5565}                & \textbf{0.4472}                & \textbf{0.3633}               \\
                               & IPW                     & 0.3942                       & \textbf{0.5560}                         & \textbf{0.4464}                         & \textbf{0.3625}                        \\
                               & CVar                    & 0.3933                       & 0.5537                         & 0.4449                         & 0.3617                        \\
                               & Rerank                  & 0.3919                       & 0.5478                         & 0.4435                         & 0.3612                        \\
                               & EASE                    & 0.3930                       & 0.5541                         & 0.4448                         & 0.3613                        \\ 
                            & Causal & 0.3551 & 0.5034 & 0.4024 & 0.3233 \\
                            & Post & 0.3927 & 0.5525 & 0.4448 & 0.3612 \\
                            & MP                    &          0.1587             &        0.2743                &    0.1749                      &           0.1161              \\                                  \cmidrule(lr){1-6}
\multicolumn{2}{c}{Standard Deviation}           & \multicolumn{4}{c}{$\pm 0.0010$}\\
\midrule
\multirow{6}{*}{Million Songs} & \system                    & \textbf{0.3915}            & \textbf{0.5116}            & \textbf{0.4290}           & \textbf{0.3341}           \\
                               & IPW                     & \textbf{0.3909}                     & 0.5099                     & \textbf{0.4290}                    & \textbf{0.3340}                    \\
                               & CVar                    & 0.3839                     & 0.5070                     & 0.4240                    & 0.3268                    \\
                               & Rerank                  & 0.3896                     & 0.5062                     & 0.4278                    & \textbf{0.3339}                    \\
                               & EASE                    & 0.3898                     & 0.5084                     & 0.4279                    & \textbf{0.3339}                    \\
                               & Causal        & 0.2361\\ 
                               & MP                    &          0.0582              &        0.0986                &    0.0680                      &           0.0427              \\                                         
                               \cmidrule(lr){1-6}
\multicolumn{2}{c}{Standard Deviation}             & \multicolumn{4}{c}{$\pm 0.0010$}\\ \bottomrule
\end{tabular}
\caption{We report the performance comparison between five different methods here. In the table, $\pm$ represents the std. deviation of the 10 repeated runs on separate test sets. Due to space limit, we only report NGCG@100. NDCGs@50 and NDCGs@20 share similar trends as Recalls.}
\vskip -0.4in
\label{tab:performance}
\end{table}

==> figures/table_coverage.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table}[t]
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{Dataset}       & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Coverage@k}                    \\
\cmidrule{3-5}
                               &                         & Top 100       & Top 50        & Top 20        \\
\midrule
\multirow{6}{*}{Movie Lens}    & \system                    & \textbf{1793} & \textbf{1052} & \textbf{530}  \\
                               & IPW                     & 1531          & 972           & 519           \\
                               & CVar                    & 1488          & 940           & 502           \\
                               & Rerank                  & 1718          & 948           & 490           \\
                               & EASE                    & 1461          & 922           & 489           \\
                               & CAUSAL                  & 1084          & 417           & 259           \\
                               & POST   &        1586 &  922 & 489 \\
                               & MP          &  100          &    50        &    20  \\  
                        \cmidrule(lr){1-5}
\multicolumn{2}{c}{Standard Deviation}                                  & $\pm 10$      & $\pm 5$       & $\pm 2$       \\
\midrule
\multirow{6}{*}{Netflix Prize}  & \system                    & \textbf{1968} & \textbf{1256} & \textbf{694}  \\
                               & IPW                     & 1802          & 1179          & 670           \\
                               & CVar                    & 1795          & 1177          & 667           \\
                               & Rerank                  & 1950          & 1190          & 655           \\
                               & EASE                    & 1762          & 1153          & 654           \\
                               & CAUSAL & 1084 & 738 & 417\\
                               & POST & 1759 & 1155 & 654 \\
                               & MP          &  100          &    50        &    20  \\                    
\cmidrule(lr){1-5}
\multicolumn{2}{c}{Standard Deviation}                                  & $\pm 6$       & $\pm 4$       & $\pm 2$       \\  
\midrule
\multirow{6}{*}{Million Song}  & \system                    & \textbf{6569} & \textbf{3692} & \textbf{1625}          \\
                               & IPW                     & 6466          & 3673          & \textbf{1626} \\
                               & CVar                    & 6337          & 3556          & 1567          \\
                               & Rerank                  & 6368          & 3624          & 1609          \\
                               & EASE                    & 6304          & 3623          & 1609      \\
                               & CAUSAL                  & 2513 &  &  \\          
                               & MP          &  100          &    50        &    20  \\                                       
\cmidrule(lr){1-5}
\multicolumn{2}{c}{Standard Deviation}                                  & $\pm 9$       & $\pm 5$       & $\pm 2$       \\
\bottomrule            
\end{tabular}
\caption{We report the coverage for five different methods in this Table. Here, $\pm$ represents the standard deviation of the coverage number of 100 users. For example, on Movie Lens, there are 10000 users in the test set. We fixed the order of user list for all the method. We split them as chunks of 100 users. We report the mean  coverage and the standard deviation for each dataset excluding baseline MP. Best results within one standard deviation are highlighted. }
\label{tab:coverage}
\vskip -0.35in
\end{table}



==> figures/table_item_perf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Dataset}       & \multirow{2}{*}{Method} & \multicolumn{3}{c}{Item Recall@k} & \multirow{2}{*}{Improve(\%)} \\   \cmidrule(lr){3-5}
                               & \multicolumn{1}{c}{} & 100       & 50        & 20        &                          \\
\midrule                            
\multirow{6}{*}{Movie Lens}    & \system                 & \textbf{0.0465}    & \textbf{0.0294}    & \textbf{0.0146}    & \textbf{13.3\%}                 \\
                               & IPW                  & 0.0433    & 0.0270     & 0.0131    & 4.4\%                 \\
                               & CVaR                 & 0.0426    & 0.0262    & 0.0127    & 2.0\%                 \\
                               & Rerank               & 0.0419    & 0.0257    & 0.0123    & 0.0\%                        \\
                               & EASE                 & 0.0419    & 0.0257    & 0.0123    & -                      \\ % 0.0799
                               & Causal               & 0.0143  & 0.0083     & 0.0041  & -                        \\ % 0.0267
                               & MP                 & 0.0067    &  0.0035    &  0.0016   & -                      \\                               
\midrule    
\multirow{6}{*}{Netflix Prize} & \system                 & \textbf{0.0958}    & \textbf{0.0631}    & \textbf{0.0342}    & \textbf{23.9\%}                 \\
                               & IPW                  & 0.0833    & 0.0526    & 0.0269    & 4.5\%                 \\
                               & CVaR                 & 0.0842    & 0.0532    & 0.0271    & 5.6\%                 \\
                               & Rerank               & 0.0802    & 0.0502    & 0.0252    & -0.1\%                 \\
                               & EASE                 & 0.0804    & 0.0502    & 0.0252    & -                       \\
                               & MP                 & 0.0083    &  0.0044   &  0.0019   & -                      \\                                                     
\midrule    
\multirow{6}{*}{Million Song}  & \system                 & \textbf{0.248}     & \textbf{0.203}     & \textbf{0.143}    & \textbf{1.2\%}                 \\
                               & IPW                  & 0.246     & 0.202     & 0.142    & 0.4\%                 \\
                               & CVaR                 & 0.240      & 0.192     & 0.131     & -0.4\%                 \\
                               & Rerank               & 0.244     & 0.201     & 0.141     & -0.2\%                 \\
                               & EASE                 & 0.245     & 0.201     & 0.141    & -   \\ 
                               & MP                   &  0.003  & 0.002   &  0.001  & -   \\
\cmidrule(lr){1-6}
\multicolumn{2}{c}{Standard Deviation}                 & \multicolumn{3}{c}{$\pm 0.0004$} & \\                                          
\bottomrule                               
\end{tabular}
\caption{In this table, we report the performance by Item Recall@k. This metric excludes the popularity bias and better reflects the effectiveness of different methods. We also report the average improvement of each method compared to the base recommender EASE.}
\label{tab:perf_item}
\vskip -0.4in
\end{table}
